Modeling Context With Linear Attention for Scalable Document-Level Translation

Document-level machine translation leverages inter-sentence dependencies to produce more coherent and consistent translations. However, these models, predominantly based on transformers, are difficult to scale to long documents as their attention layers have quadratic complexity in the sequence length. Recent efforts on efficient attention improve scalability, but their effect on document translation remains unexplored. In this work, we investigate the efficacy of a recent linear attention model by Peng et al. (2021) on document translation and augment it with a sentential gate to promote a recency inductive bias. We evaluate the model on IWSLT 2015 and OpenSubtitles 2018 against the transformer, demonstrating substantially increased decoding speed on long sequences with similar or better BLEU scores. We show that sentential gating further improves translation quality on IWSLT.

==> ARR [Oct 21] → [June 22] → EMNLP findings 2022 - RFA for Doc MT_arXiv/math_commands.tex <==

\usepackage{amsmath,amsfonts,bm}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\mathbf{0}}}
\def\vone{{\mathbf{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\mathbf{a}}}
\def\vb{{\mathbf{b}}}
\def\vc{{\mathbf{c}}}
\def\vd{{\mathbf{d}}}
\def\ve{{\mathbf{e}}}
\def\vf{{\mathbf{f}}}
\def\vg{{\mathbf{g}}}
\def\vh{{\mathbf{h}}}
\def\vi{{\mathbf{i}}}
\def\vj{{\mathbf{j}}}
\def\vk{{\mathbf{k}}}
\def\vl{{\mathbf{l}}}
\def\vm{{\mathbf{m}}}
\def\vn{{\mathbf{n}}}
\def\vo{{\mathbf{o}}}
\def\vp{{\mathbf{p}}}
\def\vq{{\mathbf{q}}}
\def\vr{{\mathbf{r}}}
\def\vs{{\mathbf{s}}}
\def\vt{{\mathbf{t}}}
\def\vu{{\mathbf{u}}}
\def\vv{{\mathbf{v}}}
\def\vw{{\mathbf{w}}}
\def\vx{{\mathbf{x}}}
\def\vy{{\mathbf{y}}}
\def\vz{{\mathbf{z}}}
\def\vphi{{\boldsymbol{\phi}}}
\def\valpha{{\boldsymbol{\alpha}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\mathbf{A}}}
\def\mB{{\mathbf{B}}}
\def\mC{{\mathbf{C}}}
\def\mD{{\mathbf{D}}}
\def\mE{{\mathbf{E}}}
\def\mF{{\mathbf{F}}}
\def\mG{{\mathbf{G}}}
\def\mH{{\mathbf{H}}}
\def\mI{{\mathbf{I}}}
\def\mJ{{\mathbf{J}}}
\def\mK{{\mathbf{K}}}
\def\mL{{\mathbf{L}}}
\def\mM{{\mathbf{M}}}
\def\mN{{\mathbf{N}}}
\def\mO{{\mathbf{O}}}
\def\mP{{\mathbf{P}}}
\def\mQ{{\mathbf{Q}}}
\def\mR{{\mathbf{R}}}
\def\mS{{\mathbf{S}}}
\def\mT{{\mathbf{T}}}
\def\mU{{\mathbf{U}}}
\def\mV{{\mathbf{V}}}
\def\mW{{\mathbf{W}}}
\def\mX{{\mathbf{X}}}
\def\mY{{\mathbf{Y}}}
\def\mZ{{\mathbf{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\operatorname{softmax}}
\newcommand{\mlp}{\operatorname{MLP}}
\newcommand{\attn}{\operatorname{attn}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} %

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> ARR [Oct 21] → [June 22] → EMNLP findings 2022 - RFA for Doc MT_arXiv/sections/01_intro.tex <==

\section{Introduction} \label{sec:intro}
Sentence-level neural machine translation has seen significant recent progress~\cite{Bahdanau2015, vaswani2017}. A move to document-level 
translation opens the possibility of using inter-sentential context at the scale of paragraphs, documents, or even whole books~\cite{lopes-etal-2020-document,ma2021comparison,maruf2021survey}. This opens up new research
avenues to improve translation and its evaluation for more consistent anaphora resolution and 
discourse coherence~\cite{bawden-etal-2018-evaluating,muller-etal-2018-large,voita-etal-2019-good}.

Transformers have enabled state-of-the-art results for sentence-level translation~\cite{vaswani2017,chen-etal-2018-best,wang-etal-2019-learning} and this success has made them the default architecture for document translation.
However, they do not scale well in the sequence length due to the quadratic complexity of attention
and hence are computationally prohibitive to apply to long text. %
Alternative architectures exist, but
most still have quadratic complexity~\cite{zhang-etal-2018-improving,voita-etal-2019-good} and/or have extra modules that further add to the inference cost \cite{tu2017learning,zhang-etal-2018-improving,miculicich-etal-2018-document,donato-etal-2021-diverse}.


By reducing asymptotic complexity, recent work on efficient attention may pave the way for long text generation.
However, these methods' suitability for document translation requires further investigation:
some do not focus on decoding speed~\citep[\emph{i.a.}]{guo-etal-2019-star,child19,Kitaev2020Reformer,wang2020linformer}, while others' speedup and quality impact for document translation remains unknown~\citep[\emph{i.a.}]{kasai2021finetuning,schlag2021linear,ma2021luna,choromanski2021rethinking}. %
In this work, we consider random feature attention (RFA; \citealp{peng2021rfa}), a representative first model with established accuracy and efficiency in sentence-level translation.
With few additional parameters, it approximates softmax attention in linear time and space with recurrent computations.
We explore its effectiveness for document translation %
and find substantial decoding speedup over a transformer with similar or improved BLEU. 
We also equip RFA with a sentential gate, injecting a recency inductive bias tailored to representing document context.%

Our main contributions are: (i) we study the efficacy of RFA for document translation; 
(ii) we validate that RFA is competitive with a transformer \rev{but substantially faster} on long documents;
(iii) we augment RFA with a sentential gate designed to promote a recency bias, which brings
a 0.5 BLEU improvement on IWSLT~\cite{Cettolo2015TheI2}. 
To encourage future research, we  release our code.\footnote{\url{https://github.com/ZhaofengWu/rfa-doc-mt}\label{fn:code}}




==> ARR [Oct 21] → [June 22] → EMNLP findings 2022 - RFA for Doc MT_arXiv/sections/02_task.tex <==
\section{Background} \label{sec:doc-mt}


\begin{figure}[t]
\centering
\includegraphics[width=0.46\textwidth]{images/sliding-window.pdf}
\caption{\label{fig:sliding-window} The concatenation model for document translation with a sliding window of length $L=4$. Every window is translated in its entirety, but only the last translated sentence is used for evaluation. The purple bars denote the sentence separator token.
}
\end{figure}




Standard machine translation independently translates each sentence.
Document translation leverages additional source and target context to produce more coherent translation, improving lexical choice and ambiguity resolution~\cite{voita-etal-2019-good}.

\paragraph{The Concatenation Model.}
Recent studies found that the concatenation model that directly translates the source document
to the target document (or a multi-sentence window) with a single encoder-decoder model performs well~\cite{tiedemann-scherrer-2017-neural,ma2021comparison}, especially on large datasets~\cite{junczysdowmunt2019microsoft}. Figure~\ref{fig:sliding-window} illustrates this model combined with sliding window decoding, which we adopt in this work.



\paragraph{Scalability of Attention.} 
In machine translation, transformers have three types of attention: encoder self-attention, cross attention, and causal attention. %
In each, every query $\vq_t$ is dotted with all keys $\{\vk_i\}$ to obtain the attention weights, with which a weighted average of the values $\{\vv_i\}$ is calculated:
\begin{align}\label{eq:attention}
\begin{split}
  \hspace{-1mm}\operatorname{attn}\left(\vq_t,\{\vk_i\},\{\vv_i\}\right)=\sum_{i=1}^{N}
    \frac{\exp\left(\vq_t \cdot \vk_i \right)}
    {\sum_{j=1}^{N}\exp\left(\vq_t \cdot \vk_{j} \right)}\vv_i^\top \nonumber
\end{split}
\end{align}
\noindent where $N$ is the sequence length. This pairwise interaction incurs quadratic overhead
in $N$, which is inefficient for the long text sequences in the concatenation model. 
This particularly impacts cross and causal attention at decoding time, which cannot be parallelized~\citep{kasai2021finetuning}.\footnote{As an example, IWSLT has a $\approx80$ sequence length with a window size of 4 (Table~\ref{tab:dataset-stats}, appendix).} %


==> ARR [Oct 21] → [June 22] → EMNLP findings 2022 - RFA for Doc MT_arXiv/sections/03_model.tex <==
\section{Scalable Document-Level Translation}

\begin{figure}[t]
\centering
\includegraphics[width=0.46\textwidth]{images/gating.pdf}
\caption{\label{fig:gating} Our sentential gating mechanism. $e_1$ and $e_4$ are at the beginnings of two sentences.
}
\end{figure}



We test RFA %
as a linear time and space model to improve the efficiency of document translation. %
We also augment it with a sentential gate to circumvent capacity constraints that come with a long context by injecting a recency inductive bias.
\subsection{Random Feature Attention}
RFA approximates the softmax attention $\operatorname{attn}\left(\vq_t,\{\vk_i\},\{\vv_i\}\right)$ in linear time and space:
\begin{align}
    \textsc{Rfa}\left(\vq_t,\{\vk_i\},\{\vv_i\}\right)=\frac{\boldsymbol{\phi}\left(\vq_t\right) \cdot \mS_t}
    {\boldsymbol{\phi}\left(\vq_t\right) \cdot \vz_t}. \nonumber
\end{align} 
\rev{The randomized nonlinear transformation $\vphi(\cdot)$
is constructed so that $\exp(\vx \cdot \vy)\approx\vphi(\vx)\cdot\vphi(\vy)$~\cite{rahimi2009rff}.} $\mS$, $\vz$ summarize keys and values. We use RFA in cross and causal attention, which are the most impactful for speed and memory, so $\vq_t$ is always from the target sequence. 
In cross attention, $\mS$ and $\vz$ represent the source sequence and are constant for all query positions $t$: $\mS_t = \sum_{i=1}^{N} \boldsymbol{\phi}(\vk_i)\vv_i^\top$ and $\vz_t = \sum_{i=1}^{N} \boldsymbol{\phi}(\vk_i)$.
In causal attention, they represent the target prefix ${i\le t}$: $\mS_t = \sum_{i=1}^{t} \boldsymbol{\phi}(\vk_i)\vv_i^\top = \mS_{t-1} + \boldsymbol{\phi}\left(\vk_t\right)\vv_t^\top$ and $\vz_t = \sum_{i=1}^{t} \boldsymbol{\phi}(\vk_i) = \vz_{t-1} + \boldsymbol{\phi}\left(\vk_t\right)$. 
These recurrent computations are analogous to an RNN with $\mS_t$ and $\vz_t$ as hidden states at step $t$ and enable constant computation per timestep.
RFA serves as a drop-in replacement for attention in transformers.
The encoder and other modules, e.g., feed-forward layers, remain the same.
We refer the reader to \citet{peng2021rfa} for more details on RFA.


\subsection{Sentential Gating} \label{sec:gating}
\citet{schlag2021linear} noted, under the lens of fast weight programmers~\cite{Schmidhuber:91fastweights,schmidhuber1992learning,schmidhuber1993reducing}, that accumulating memory in a purely additive manner, \rev{like $\mS$ and $\vz$} above, will reach a capacity limitation with sequences longer than the size of $\vphi$. %
This is particularly an issue in document-level translation due to the long sequences.

Nevertheless, document translation admits a natural solution to this constraint: inspired by gated RNNs~\citep[\emph{i.a.}]{cho-etal-2014-learning}, we augment RFA with a sentence-level gate to enable dynamic control of
contextual information from the current and previous sentences, and to allow the model to selectively forget about the history to circumvent the capacity constraint. This is illustrated in Figure~\ref{fig:gating}.
For the $t$th word with representation $\ve_t$, we compute a forget gate using the sentence separator token:
\begin{align}
\begin{split}
    f_t &= 
    \begin{cases}
        \sigma( \vw_f\cdot \ve_{t-1}+ b_f) & \text{if }x_t\text{ starts a sentence}\\
        1 & \text{otherwise}\\
    \end{cases}\\
    \mS_t &= f_t \; \mS_{t-1} + \boldsymbol{\phi}\left(\vk_t\right)\vv_t^\top \\
    \vz_t &= f_t \; \vz_{t-1} + \boldsymbol{\phi}\left(\vk_t\right)  \nonumber
\end{split}
\end{align}
$\sigma$ is the sigmoid function; $\vw_f$ and $b_f$ are learned parameters.
The context is decayed when a new sentence starts, and the decay coefficient is reused for all tokens in the same sentence.
Specifically, each sentence $j$ assigns a weight $0 < \prod_{i=\textsc{start}(j')+1}^{\textsc{start}(j)} f_i < 1$ when attending to a previous sentence $j'$, where $\textsc{start}(\cdot)$ is the first token in a sentence.
This introduces an inductive bias that, intuitively, previous sentences are less important in translation, and their representations are decayed.


\paragraph{Relation to Prior Work.} While gating is common in RNNs, it is less clear how it applies to transformers.
\citet{miculicich-etal-2018-document} gated at the sentence level, though hierarchically, while we gate recurrently. 
Ours also contrasts with the per-token gating of \citet{peng2021rfa} which they found ineffective for machine translation.
These two works also take a weighted average of the previous and current sentences while we only decay the former. We show our variant performs better in \S\ref{sec:results}.
\citet{schlag2021linear} used a gate that explicitly models memory removal, but also at the token level.


==> ARR [Oct 21] → [June 22] → EMNLP findings 2022 - RFA for Doc MT_arXiv/sections/04_setup.tex <==
\section{Experimental Setup} \label{sec:setup}



\paragraph{Datasets and Evaluation.} We experiment with the IWSLT 2015 Chinese-to-English (zh-en) dataset~\cite{Cettolo2015TheI2} with multilingual TED talk captions and the OpenSubtitles2018 English-to-Russian (en-ru) dataset~\cite{lison-etal-2018-opensubtitles2018} with movie and TV subtitles.
We measure document-level BLEU~\cite{papineni-etal-2002-bleu} with SacreBLEU~\cite{post-2018-call}.\footnote{We use fairseq's default setting which has hash \texttt{case.mixed+numrefs.?+smooth.exp+tok.none\\+version.1.5.0} with standalone 13a-tokenization.}
To quantify discourse consistency,
we also use the test sets by \citet{voita-etal-2019-good} based on OpenSubtitles.
We introduce these datasets and their statistics in more detail in \S\ref{sec:dataset-and-processing-details}.


\paragraph{Data Processing.} %
We process each document with a stride-one sliding window of $L$ sentences to obtain our training set.
Following \citet{voita-etal-2019-good} and \citet{ma2021comparison}, we experiment with $L=1$, the sentence-level baseline, and $L=4$. During inference, we use the last translated sentence in each window for evaluation. %
For a more granular analysis, we consider $L\in \{1,2,3,4\}$ for consistency experiments.
More details are in \S\ref{sec:dataset-and-processing-details}.


\paragraph{Model Settings.} We compare RFA and transformer with the concatenation model. For RFA, we experiment with no gating (\textbf{RFA}) and sentential gating (\textbf{RFA-sgate}). To compare our decaying gate choice with prior work (\S\ref{sec:gating}), we run a sentential-gated RFA that takes a weighted average of previous and current text (\textbf{RFA-sgate-avg}). We mostly default to fairseq hyperparameters~\cite{ott2019fairseq}, most suitable for the $L=1$ transformer (\S\ref{sec:hyperparameters}).


==> ARR [Oct 21] → [June 22] → EMNLP findings 2022 - RFA for Doc MT_arXiv/sections/05_results.tex <==
\section{Results} \label{sec:results}







    






\begin{table}[t!]
    \centering
    \aboverulesep=0ex
    \belowrulesep=0ex
    \renewcommand{\arraystretch}{1.2}
    \setlength{\tabcolsep}{6.5pt}
    \begin{tabular}{@{} l @{\hspace{3pt}} c@{\hspace{5pt}}c @{\hspace{5pt}} c@{\hspace{5pt}}c @{}}
        \toprule
        & \multicolumn{2}{c}{\textbf{IWSLT}} & \multicolumn{2}{c}{\textbf{Subtitles}} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5}
        \textbf{Window Size $L$} & \textbf{1} & \textbf{4} & \textbf{1} & \textbf{4} \\
        \midrule
        \midrule
        Transformer & 31.7 & 30.4 & 32.6 & 33.1 \\
        \midrule
        RFA & 31.0 & \textbf{30.7} & \textbf{32.9} & \textbf{33.2} \\
        RFA-sgate-avg & --- & \textbf{30.8} & --- & 33.0 \\
        RFA-sgate & --- & \textbf{31.2} & --- & \textbf{33.2} \\
        \bottomrule
    \end{tabular}
    \caption{\label{tab:bleu} BLEU on IWSLT and OpenSubtitles test sets. Bold scores outperform the transformer. %
    }
\end{table}

\begin{figure}[t]
\centering
\includegraphics[width=0.43\textwidth]{images/consistency.png}
\caption{\label{fig:consistency} Model performance on the consistency test set, broken down into phenomena. Transformer and RFA are tested with window sizes from 1 to 4. We compare with the baselines in \citet{voita-etal-2019-good} and \citet{ma2021comparison} corresponding to our Transformer $L=4$.
}
\end{figure}

\begin{figure}[t]
\centering
    \includegraphics[width=0.45\textwidth]{images/speedup.png}
\caption{\label{fig:speedup} \rev{RFA's inference speedup over the transformer in the number of decoded tokens per second. Each sentence has $\approx20$ tokens (Table~\ref{tab:dataset-stats}, appendix).}
}
\end{figure}


\paragraph{BLEU Scores.} Table~\ref{tab:bleu} shows BLEU scores on IWSLT and OpenSubtitles. 
The sentence-level transformer has the highest IWSLT BLEU, possibly due to defaulting to fairseq hyperparameters optimized for this setting.
With $L=4$, RFA performs slightly better than the transformer, showing suitability for long-text translation. %
Gated RFA further brings a 0.5 BLEU improvement, confirming its utility, but gating has no effect on OpenSubtitles. We hypothesize that with only $\approx$10 tokens per sentence, half of the average length of IWSLT (Table~\ref{tab:dataset-stats}, appendix), \rev{the capacity constraint~\cite{schlag2021linear} is less severe and thus gating would be less useful}.
Our gate also outperforms the averaging variant in \citet{miculicich-etal-2018-document} and \citet{peng2021rfa}, validating its effect on document translation.
Aligning with prior findings \cite{voita-etal-2019-good,ma2021comparison}, longer contexts do not clearly lead to better BLEU, though it improves consistency metrics, to which we turn next.








\paragraph{Discourse Consistency Scores.}

Figure~\ref{fig:consistency} plots the consistency scores in four phenomena for RFA, \rev{including our gated variants}, and the transformer baseline from \citet{voita-etal-2019-good} and \citet{ma2021comparison}. %
We also re-implement this transformer model to control confounding factors in implementation details and to extrapolate to $L<4$, which they did not thoroughly explore.
We compare to a baseline \rev{that chooses its prediction randomly from candidate translations; see \S\ref{sec:dataset-and-processing-details} for details.}

Translating with longer contexts almost always yields better consistency, which is also a setting where RFA achieves better speedup, shown later.
\rev{Gating does not have a clear benefit, aligning with OpenSubtitles' BLEU pattern.}
RFA slightly underperforms the transformer on ellipsis.
We hypothesize that the direct query-key interaction in softmax attention is more suitable for precise long-distance information extraction, sometimes required for consistency, than the RFA approximation. 
\rev{
On lexical cohesion, transformer shows a large variance: with the same architecture and size,
\citet{ma2021comparison}, \citet{voita-etal-2019-good}, and our implementation of $L=4$ transformer
achieve drastically different scores.
\citet{voita-etal-2019-good}'s implementation and RFA fail to outperform the random baseline on this phenomenon.
}
\rev{Reliable evaluation of lexical cohesion, and the related task of word sense disambiguation, are known to be challenging in document translation: models tend to rely on dataset artifacts but not the context, and the attention of well-performing models poorly aligns with the ground-truth required for disambiguation~\citep{kim-etal-2019-document,emelin-etal-2020-detecting,yin-etal-2021-context}.}


\paragraph{Speed.}
\rev{We confirmed the observation from prior work that longer context boosts translation consistency and sometimes BLEU.}
It would be exciting to examine this trend with $L>4$, but to our knowledge, it has little existing evaluation data.
We therefore measure decoding efficiency with a synthetic experiment by decoding for all $L$ with the same trained model.  We focus only on efficiency here, not quality.
We measure the number of decoded tokens per second over the forward pass time on IWSLT's test set.
We follow \citet{ott-etal-2018-scaling} and cache $\vk$ and $\vv$ 
for our \emph{baseline} which substantially increases its speed.
More details are in \S\ref{sec:benmark-details}.

Figure~\ref{fig:speedup} shows RFA's speedup relative to the transformer. \rev{On GPU, without document context, RFA is slower, likely due to its random matrix overhead. Nevertheless, its speed over the transformer roughly linearly increases, agreeing with the theory, up to $2.09\times$ on our longest tested context $L=15$.
RFA enables an even more substantial speedup on other device types. For sentence-level translation, RFA is in fact faster than the transformer by 1.58$\times$ on CPU, and, as \citet{peng2021rfa} reported, by 1.8--1.9$\times$ on TPU. At $L=15$, its CPU speedup increases to 19.2$\times$. Therefore, depending on the use case, such as when decoding on edge devices, RFA could be even more favorable. Furthermore, we used the same batch size between RFA and the transformer. With lower memory complexity, RFA accommodates a larger batch size and in practice achieve a more significant speedup. For example, at $L=15$ on GPU, we found that RFA allows a 5$\times$ batch size and enables a more than $7\times$ speedup.}

\rev{RFA's superior speed makes it an attractive choice to leverage very long contexts. Nevertheless, we are merely extrapolating the utility of long context from our experiments. The extent to which it really helps needs to be verified by future curated test sets. We hope the demonstration of our model's ability to efficiently and effectively process document context could catalyze such efforts.}








==> ARR [Oct 21] → [June 22] → EMNLP findings 2022 - RFA for Doc MT_arXiv/sections/06_conclusion.tex <==
\section{Conclusion}

We explored the effectiveness of random feature attention on document translation. Our model substantially improves its speed over a transformer with similar or improved BLEU. Our sentential gate also proves effective, especially on long sequences. While our model may potentially be used to produce toxic or fake information, it also enables more efficient detectors toward such content.
